Securing 5G Bootstrapping: A Two-Layer IBS Authentication Protocol

The lack of authentication during the initial bootstrapping phase between cellular devices and base stations allows attackers to deploy fake base stations and send malicious messages to the devices. These attacks have been a long-existing problem in cellular networks, enabling adversaries to launch denial-of-service (DoS), information leakage, and location-tracking attacks. While some defense mechanisms are introduced in 5G, (e.g., encrypting user identifiers to mitigate IMSI catchers), the initial communication between devices and base stations remains unauthenticated, leaving a critical security gap. To address this, we propose E2IBS, a novel and efficient two-layer identity-based signature scheme designed for seamless integration with existing cellular protocols. We implement E2IBS on an open-source 5G stack and conduct a comprehensive performance evaluation against alternative solutions. Compared to the state-of-the-art Schnorr-HIBS, E2IBS reduces attack surfaces, enables fine-grained lawful interception, and achieves 2x speed in verification, making it a practical solution for securing 5G base station authentication.

==> sections/discussion.tex <==
\noindent\textbf{Relay attacks.} Our time-bounding technique for relay attack protection is a best-effort approach. It cannot completely thwart relay attacks, rather it raises the bar for the attackers. A precise defense for relay attack would require a sophisticated approach with major changes in the protocol (e.g., including new messages) and a precise estimation of the timing/latency of message transmission and calculation, environmental interference, and hardware used by base stations and
cellular devices. We leave this for future work.

\noindent\textbf{Emergency services.} According to 3GPP~\cite{3GPP:33.501}, devices without SIM/USIM/eSIM do not perform authentication with the network for emergency calls/SMSs. To authenticate base stations in cases where a SIM was installed in the cellular device but was subsequently removed, the device can use a cached copy of the public key of their network operator's core-PKG in the UICC. We do not support base station authentication if a SIM was never inserted on a cellular device.

\noindent\textbf{UICC vs. UE.} 3GPP recommends either UICC or UE for public key encryption of SUPI~\cite{3GPP:33.501}. We, therefore, envision the implementation of signature verification at UE.

\noindent\textbf{Backward compatibility.} Our solution is backward-compatible since base stations only include the information required for our scheme in the \emph{optional fields} of SIB messages. Legacy devices ignore those fields and authentication.
